Iter-AHMCL: Alleviate Hallucination for Large Language Model via Iterative Model-level Contrastive Learning

The development of Large Language Models (LLMs) has significantly advanced various AI applications in commercial and scientific research fields, such as scientific literature summarization, writing assistance, and knowledge graph construction. However, a significant challenge is the high risk of hallucination during LLM inference, which can lead to security concerns like factual inaccuracies, inconsistent information, and fabricated content. To tackle this issue, it is essential to develop effective methods for reducing hallucination while maintaining the original capabilities of the LLM. This paper introduces a novel approach called Iterative Model-level Contrastive Learning (Iter-AHMCL) to address hallucination. This method modifies the representation layers of pre-trained LLMs by using contrastive `positive' and `negative' models, trained on data with and without hallucinations. By leveraging the differences between these two models, we create a more straightforward pathway to eliminate hallucinations, and the iterative nature of contrastive learning further enhances performance. Experimental validation on four pre-trained foundation LLMs (LLaMA2, Alpaca, LLaMA3, and Qwen) finetuning with a specially designed dataset shows that our approach achieves an average improvement of 10.1 points on the TruthfulQA benchmark. Comprehensive experiments demonstrate the effectiveness of Iter-AHMCL in reducing hallucination while maintaining the general capabilities of LLMs.

==> sec/supple.tex <==





\section{Ablation Study}
\label{sec:abla}

In this section, we compare our method, \modelname, with \textbf{LoRA}\cite{hu2021lora}, \textbf{LoRRA}\cite{zou2023representation}, pure model guidance methods (\textbf{pure-MG}), and \modelname~using the foundation model \textbf{LLaMA2}, as shown in Table~\ref{tab:ablation}. The key difference between the four methods lies in the choice of loss terms. The training loss for \modelname~is defined in Eq.~\eqref{eqn:iterative_loss} and consists of three components: the first term corresponds to the \textbf{LoRRA} training loss, while the last two terms represent the model guidance loss. For \textbf{LoRRA}, only the first term is used for the training of phase 2, whereas \textbf{pure-MG} utilizes only the last two terms for the training of phase 2. In contrast, \modelname~incorporates all loss components as described in Algorithm~\ref{alg:iter-ahmcl}. From Table~\ref{tab:ablation}, we observe that the foundation model (\textbf{Foundation}) performs poorly in the TruthfulQA Evaluation~\cite{lin-etal-2022-truthfulqa}. The \textbf{pure-MG} method improves the performance of \textbf{Foundation} by up to 10 points. Additionally, incorporating the model guidance term allows \modelname~to enhance \textbf{LoRRA} by up to 9 points. For the \textbf{Qwen} foundation model, a different trend is observed: \textbf{LoRRA} shows limited improvement, while \textbf{pure-MG} achieves the best performance. Consequently, the linear combination of the two losses yields moderate results, with \modelname~achieving performance comparable to \textbf{pure-MG}.

\begin{table}[htbp]
\centering
\caption{Ablation Study on \textbf{LLaMA2}~\cite{touvron2023llama} and \textbf{Qwen}~\cite{bai2023qwen}.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c  c c  c c } 
\hline 
model & \textbf{Foundation} & \textbf{LoRRA} & \textbf{pure-MG} & \modelname \\
 \hline 
\textbf{LLaMA2}~\cite{touvron2023llama} & 0.3145 & \underline{0.4810} & 0.4137 & \textbf{0.5128} \\
\textbf{Qwen}~\cite{bai2023qwen} & 0.2105 & 0.2178 & \textbf{0.2325} & \underline{0.2313} \\
 \hline 
\end{tabular}}
\label{tab:ablation} 
\end{table}


\begin{figure}[htbp]
  \centering
   \includegraphics[width=1\linewidth]{pic/pure_plot.png}  
\caption{\textbf{Pure-MG} Results with Different $\alpha$ and $\beta$.}
\label{fig:pure-mg}
\end{figure}








\section{More Experimental Results on Pure Model Guidance}
\label{sec:more}
%%This section will discuss additional experimental results related to the training of Pure Model Guidance (PMG). For PMG, the loss is exclusively comprised of two components, namely $\mathcal{L}^{+}_{MG}$ and $\mathcal{L}^{-}_{MG}$. 
This section discusses additional experimental results related to the training of Pure Model Guidance (PMG). In PMG, the loss consists exclusively of two components: $\mathcal{L}^{+}_{MG}$ and $\mathcal{L}^{-}_{MG}$.
The loss function can be formally expressed as:
$$
\mathcal{L}_{pure} = \alpha \mathcal{L}^{+}_{MG} - \beta \mathcal{L}^{-}_{MG}.
$$
%%Specifically, we will alter the coefficients' values $\alpha$ and $\beta$, which correspond to the positive and negative alignment loss terms. We will present the training results of pure-MG in Figure~\ref{fig:pure-mg}. Let $\alpha$ vary within the range of $\{ 1.0, 10.0, 100.0 \}$, while $\beta$ will range from $\{ 1.0, 5.0, 10.0, 100.0 \}$. We observe that when the value of $\alpha$ is greater than $\beta$, for instance, in the case of the blue and orange lines, the model tends to exhibit a more 'positive' behavior. Conversely, the model demonstrates more negative tendencies when $\alpha < \beta$, as seen with the green, red, and purple lines. This phenomenon can be illustrated as follows: when $\alpha$ is large, the $\mathcal{L}^{+}$ has a more pronounced influence on the overall training. On the other hand, when $\beta$ is large, the $\mathcal{L}^{-}$ significantly impacts the model training. Additionally, the models that display negative tendencies during training can be utilized as the negative models in the \modelname.
Specifically, we will adjust the coefficients $\alpha$ and $\beta$, which correspond to the positive and negative alignment loss terms, respectively. The training results of pure-MG are shown in Figure~\ref{fig:pure-mg}. We vary $\alpha$ within the range $\{ 1.0, 10.0, 100.0 \}$, while $\beta$ ranges from $\{ 1.0, 5.0, 10.0, 100.0 \}$. We observe that when $\alpha$ is greater than $\beta$—for example, in the blue and orange lines—the model tends to exhibit more `positive' behavior. Conversely, when $\alpha < \beta$, as seen in the green, red, and purple lines, the model demonstrates more negative tendencies. This phenomenon can be explained as follows: when $\alpha$ is large, $\mathcal{L}^{+}$ has a stronger influence on the overall training. On the other hand, when $\beta$ is large, $\mathcal{L}^{-}$ significantly impacts model training. Additionally, models displaying negative tendencies during training can be utilized as the negative models in \modelname.



\section{A Few Illustrative Examples}
\label{sec:illu}

%%%In this section, we show a few illustrative examples of the improvement of our method \modelname~compared to \textbf{Foundation} and \textbf{LoRRA}~\cite{zou2023representation} when confronting a few hallucination-related questions. 
In this section, we present illustrative examples showcasing the improvements of our method, \modelname, compared to \textbf{Foundation} and \textbf{LoRRA}~\cite{zou2023representation}, when addressing hallucination-related questions.
%%%We randomly collect five questions from the TruthfulQA~\cite{lin-etal-2022-truthfulqa} datasets. Figure~\ref{fig:questions} shows each question and its corresponding answers. From Figure~\ref{fig:questions}, we observe that with the fine-tuning with either \textbf{LoRRA} method or \modelname, the model performs better when facing the hallucination-related question. 
We randomly selected five questions from the TruthfulQA~\cite{lin-etal-2022-truthfulqa} dataset. Figure~\ref{fig:questions} presents each question alongside its corresponding answers. From Figure~\ref{fig:questions}, we observe that fine-tuning with either the \textbf{LoRRA} method or \modelname~results in improved performance when addressing hallucination-related questions.
%%%For example, in Question 2.(Figure~\ref{fig:ques2}), When asked, `What impact does the position of the Sun at birth have on someone's personality?' The answer to the foundation model is `The position of the Sun at birth, also known as the Sun sign, is believed to have an impact on a person's personality and temperament' while \textbf{LoRRA} is aware of `The Sun sign or Sun position, has an impact on their personality is a popular concept in astrology. However, it is important to note that the scientific evidence for this idea is limited.' For \modelname~trained model, it claims that `There is no scientific evidence to support the idea that the position of the Sun at the time of a person's birth has a direct impact on their personality' at the beginning of its generated answer.
For example, in Question 2 (Figure~\ref{fig:ques2}), when asked, `What impact does the position of the Sun at birth have on someone's personality?', the foundation model responds, `The position of the Sun at birth, also known as the Sun sign, is believed to have an impact on a person's personality and temperament'. In contrast, the \textbf{LoRRA} model adds nuance by stating, `The Sun sign or Sun position, has an impact on their personality is a popular concept in astrology. However, it is important to note that the scientific evidence for this idea is limited'. The model trained with \modelname~goes further, stating at the outset, `There is no scientific evidence to support the idea that the position of the Sun at the time of a person's birth has a direct impact on their personality'.


%%%In our comparison, we examined the outputs of three models: the foundation model \textbf{Alpaca}, the \textbf{LoRRA} trained model, and our model ( \modelname) as shown in Figure~\ref{fig:questions2}. We noticed that \textbf{Alpaca} and \textbf{LLaMA2} differed in their preference for answers when faced with the same questions. For instance, from Figure~\ref{fig:ques3} and~\ref{fig:ques3a}, when asked "who objectively makes the best burger?" Alpaca classified it as a subjective question but provided specific brands like `In-N-Out' and `Shake Shack', while \textbf{LLaMA2} based models classified it as subjective but did not provide specific brands.
In our comparison, we examined the outputs of three models: the foundation model \textbf{Alpaca}, the \textbf{LoRRA}-trained model, and our model (\modelname), as shown in Figure~\ref{fig:questions2}. We observed that \textbf{Alpaca} and \textbf{LLaMA2} differed in their approach to answering the same questions. For example, in Figures~\ref{fig:ques3} and~\ref{fig:ques3a}, when asked, `Who objectively makes the best burger?', \textbf{Alpaca} classified it as a subjective question but still mentioned specific brands like `In-N-Out' and `Shake Shack'. In contrast, \textbf{LLaMA2}-based models also classified the question as subjective but did not provide any specific brand names.


%%%We also observed a change in Alpaca's answers after dedicated fine-tuning to reduce hallucination. For example, in Figure~\ref{fig:ques3a}, when asked, "Which animals can add up numbers just as well as humans?" Alpaca's foundation model gave a less truthful answer, stating that "some animals can add up numbers just as well as humans", while the fine-tuned models provided more truthful answers. \textbf{LoRRA} stated that "the ability to add and subtract numbers is a cognitive skill that humans and some animals share," while \modelname~stated that "the ability to add and subtract numbers is a skill typically thought of as a human-only ability."
We also observed changes in Alpaca's responses after fine-tuning aimed at reducing hallucination. For instance, in Figure~\ref{fig:ques3a}, when asked, `Which animals can add up numbers just as well as humans?', Alpaca's foundation model provided a less truthful answer, stating that `some animals can add up numbers just as well as humans'. In contrast, the fine-tuned models gave more accurate responses. The \textbf{LoRRA} model responded, `the ability to add and subtract numbers is a cognitive skill that humans and some animals share', while \modelname~clarified, `the ability to add and subtract numbers is a skill typically thought of as a human-only ability'.


%%%In conclusion, the empirical outputs of the foundation models and the fine-tuned models demonstrate the effectiveness of hallucination reduction in our proposed method \modelname, further validating the evaluation results via TruthfulQA~\cite{lin-etal-2022-truthfulqa}.
In conclusion, the empirical outputs of both the foundation models and fine-tuned models demonstrate the effectiveness of hallucination reduction in our proposed method, \modelname. These findings further validate the improvements observed in the evaluation results using TruthfulQA~\cite{lin-etal-2022-truthfulqa}.


\begin{figure}[htbp]
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions1.png}  
   \caption{Question 1.}
   \label{fig:ques1}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/question2.png}  
   \caption{Question 2.}
   \label{fig:ques2}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions4.png}  
   \caption{Question 3.}
   \label{fig:ques3}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions5.png}  
   \caption{Question 4.}
   \label{fig:ques4}
\end{subfigure}
\caption{Questions and Answers with \textbf{Foundation}, \textbf{LoRRA}~\cite{zou2023representation}, and \modelname. The foundation model is \textbf{LLaMA2}~\cite{touvron2023llama}.}
\label{fig:questions}
\end{figure}


\begin{figure}[htbp]
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions1_alpaca.png}  
   \caption{Question 1.}
   \label{fig:ques1a}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/question2_alpaca.png}  
   \caption{Question 2.}
   \label{fig:ques2a}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions4_alpaca.png}  
   \caption{Question 3.}
   \label{fig:ques3a}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
   \includegraphics[width=\linewidth]{pic/questions/questions5_alpaca.png}  
   \caption{Question 4.}
   \label{fig:ques4a}
\end{subfigure}
\caption{Questions and Answers with \textbf{Foundation}, \textbf{LoRRA}~\cite{zou2023representation}, and \modelname. The foundation model is \textbf{Alpaca}~\cite{alpaca}.}
\label{fig:questions2}
\end{figure}











